Noise Injection for__Performance Bottleneck Analysis

Bottleneck evaluation plays a crucial part in performance tuning of HPC applications, as it directly influences the search for optimizations and the selection of the best hardware for a given code. In this paper, we introduce a new model-agnostic, instruction-accurate framework for bottleneck analysis based on performance noise injection. This method provides a precise analysis that complements existing techniques, particularly in quantifying unused resource slack. Specifically, we classify programs based on whether they are limited by computation, data access bandwidth, or latency by injecting additional noise instructions that target specific bottleneck sources. Our approach is built on the LLVM compiler toolchain, ensuring easy portability across different architectures and microarchitectures which constitutes an improvement over many state-of-the-art tools. We validate our framework on a range of hardware benchmarks and kernels, including a detailedstudy of a sparse-matrix--vector product (SPMXV) kernel, where we successfully detect distinct performance regimes. These insights further inform hardware selection, as demonstrated by our comparative evaluation between HBM and DDR memory systems.

==> spmxv_ddrhbm.tex <==
\begin{wrapfigure}{l}{0.3\textwidth}
\begin{center}

\begin{tabular}[]{@{}lcc@{}}
\toprule

\textbf{Memory types} & DDR & HBM  \\
\midrule
\midrule

$q=0$ &&\\
$q=0.25$ &&\\
$q=0.5$ &&\\

 \bottomrule  
\end{tabular}

\captionof{table}{Performance of SPMXV (matrix (b)) on Sapphire Rapids for varying values of $q$. HBM performances collapse when $q$ is non-zero.}
\label{table:spmxv_ddrhbm}

\end{center}
\end{wrapfigure}
